Distributed Estimation and Control for Jamming an Aerial Target With Multiple Agents

This work proposes a distributed estimation and control approach in which a team of aerial agents equipped with radio jamming devices collaborate in order to intercept and concurrently track-and-jam a malicious target, while at the same time minimizing the induced jamming interference amongst the team. Specifically, it is assumed that the malicious target maneuvers in 3D space, avoiding collisions with obstacles and other 3D structures in its way, according to a stochastic dynamical model. Based on this, a track-and-jam control approach is proposed which allows a team of distributed aerial agents to decide their control actions online, over a finite planning horizon, to achieve uninterrupted radio-jamming and tracking of the malicious target, in the presence of jamming interference constraints. The proposed approach is formulated as a distributed model predictive control (MPC) problem and is solved using mixed integer quadratic programming (MIQP). Extensive evaluation of the system's performance validates the applicability of the proposed approach in challenging scenarios with uncertain target dynamics, noisy measurements, and in the presence of obstacles.

==> biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{savvas.png}}]%
{Savvas Papaioannou} received the B.S. degree in electronic and computer engineering in 2011 from the Technical University of Crete, Chania, Greece, the M.S. degree in electrical engineering in 2013 from Yale University, New Haven, CT, USA, and the Ph.D. degree in computer science in 2017 from the University of Oxford, Oxford, U.K. He is currently a Research Associate with the KIOS Research and Innovation Center of Excellence, University of Cyprus, Nicosia, Cyprus. His research interests include multi-agent and autonomous systems, state estimation and control, multi target tracking, probabilistic inference, Bayesian reasoning, and intelligent unmanned-aircraft vehicle (UAV) systems and applications. 
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pkolios}}]
{Panayiotis Kolios} is a Research Assistant Professor at the KIOS Research and Innovation Center of Excellence at the University of Cyprus. He received his B.Eng and Ph.D degrees in Telecommunications Engineering from King's College London in 2008 and 2011, respectively. His interests focus on both basic and applied research on networked intelligent systems. Some examples of such systems include intelligent transportation systems, autonomous unmanned aerial systems, and the plethora of cyber-physical systems that arise within the Internet of Things. Particular emphasis is given to emergency response aspects in which faults and attacks could cause disruptions that need to be effectively handled. He is an active member of IEEE, contributing to a number of technical and professional activities within the Association.
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{GEllinas}}]
{Georgios Ellinas} (M'98 - SM'07) holds a B.S., M.Sc., M.Phil., and a Ph.D. in Electrical Engineering from Columbia University. He is a Professor and the past Chair (2014-2020) of the Department of Electrical and Computer Engineering and a founding member of the KIOS Research and Innovation Center of Excellence at the University of Cyprus. Previously, he served as Associate Professor of Electrical Engineering at City College of New York (2002-2005), Senior Network Architect at Tellium Inc. (2000-2002), and Research Scientist/Senior Research Scientist at Bell Communications Research (Bellcore) (1993-2000). Prof. Ellinas is a Fellow of the IET (2019), a Senior Member of IEEE, OSA, and ACM, and a Member of the Marie Curie Fellows Association (MCFA). He has co-authored/co-edited four books on optical networks, more than 255 archived articles, conference papers, and book chapters, and he is the holder of 30 patents on optical networking. His research interests are in optical/telecommunication networks, transportation networks, IoT, and critical infrastructure systems.
\end{IEEEbiography}
